${\bf B_s\to K^{(*)} \ell\bar \nu}$, Angular Analysis, S-wave Contributions and ${\bf |V_{ub}|}$

We analyse the $\overline B_s^0\to K^+l^-\bar \nu$ and $\overline B_s^0\to K^{*+}(\to K\pi) \ell^-\bar \nu$ decays that are valuable for extracting the CKM matrix element $|V_{ub}|$. We calculate the differential and integrated partial widths in units of $|V_{ub}|^2$ based on various calculations of hadronic form factors and in particular the latest Lattice QCD calculation of the $B_s\to K^*$ form factors. For the decay $\overline B_s^0 \to K\pi \ell\bar \nu$, we formulate the general angular distributions with the inclusion of the various partial-wave $K\pi$ contributions. Using the results for the $K\pi$ scalar form factor calculated from unitarized chiral perturbation theory, we explore the S-wave effects on angular distribution variables and demonstrate that they may not be negligible, considering the high precision expected in future measurements. We also briefly discuss the impact of the S-wave $\pi\pi$ contributions in the $B^-\to \pi^+\pi^-\ell \bar \nu$ decay and provide estimates for the mode $B^-\to K^+K^-\ell \bar \nu$. The studies of these channels in future can not only be used to determine $|V_{ub}|$, but may also provide valuable information on the $K\pi$ and $\pi\pi$ phase shifts.

==> tableBrho.tex <==
\begin{table}[t]
\begin{center}
\caption{Integrated decay widths for
 $B^-\to \pi^+ \pi^-  \ell\bar  \nu$:
 $\Delta \zeta_{ \pi \pi}^{\ell} (q_l^2, q_u^2)$. 
Results are given in units of $ps^{-1}$.
The S-wave contributions are obtained 
with form factors calculated in the PQCD approach.}
\label{tab:integratedWidthBtopipi}
\begin{tabular}{cc|cccccccc}
\hline\hline
  & & S-Wave & P-Wave & Total &$f_S(\%)$  \\\hline
$\Delta \zeta_{\pi \pi}^\mu(0, 4)$
 & LFQM  & $0.068\pm 0.038 $ & $ 0.656\pm 0.137 $&$ 0.723\pm 0.176 $&$ 9.41 $\
 
  
\\
 & LCSR  & $0.068\pm 0.038 $ & $ 0.754\pm 0.128 $&$ 0.822\pm 0.166 $&$ 8.27 $\
 
  
\\
 $\Delta \zeta_{\pi \pi }^\mu(4, 8)$ 
 & LFQM  & $0.068\pm 0.038 $ & $ 0.984\pm 0.206 $&$ 1.05\pm 0.247 $&$ 6.48 $ 
\\
 & LCSR  & $0.068\pm 0.038 $ & $ 1.11\pm 0.205 $&$ 1.18\pm 0.241 $&$ 5.76 $ 
\\
$\Delta \zeta_{\pi \pi }^\mu(8, 12)$
 & LFQM  & $0.064\pm 0.036 $ & $ 1.29\pm 0.268 $&$ 1.35\pm 0.308 $&$ 4.74 $ 
\\
 & LCSR  & $0.064\pm 0.036 $ & $ 1.41\pm 0.261 $&$ 1.47\pm 0.301 $&$ 4.35 $ 
\\
$\Delta \zeta_{\pi \pi }^\mu(12, 16)$
 & LFQM  & $0.054\pm 0.03 $ & $ 1.42\pm 0.294 $&$ 1.47\pm 0.329 $&$ 3.67 $ 
\\
 & LCSR  & $0.054\pm 0.03 $ & $ 1.53\pm 0.297 $&$ 1.58\pm 0.331 $&$ 3.42 $ 
\\
$\Delta \zeta_{\pi \pi }^\mu(0, 16)$
 & LFQM  & $0.254\pm 0.143 $ & $ 4.34\pm 0.916 $&$ 4.6\pm 1.05 $&$ 5.52 $ 
\\
 & LCSR  & $0.254\pm 0.143 $ & $ 4.8\pm 0.895 $&$ 5.06\pm 1.03 $&$ 5.02 $ 
\\
\hline
 $\Delta \zeta_{\pi \pi }^\tau(m_\tau^2, 8)$
 & LFQM  & $0.069\pm 0.039 $ & $ 0.793\pm 0.166 $&$ 0.862\pm 0.205 $&$ 8. $ 
\\
 & LCSR  & $0.069\pm 0.039 $ & $ 0.92\pm 0.171 $&$ 0.988\pm 0.211 $&$ 6.98 $ 
\\
$\Delta \zeta_{\pi \pi }^\tau(8, 12)$
 & LFQM  & $0.074\pm 0.042 $ & $ 1.15\pm 0.241 $&$ 1.22\pm 0.288 $&$ 6.07 $ 
\\
 & LCSR  & $0.074\pm 0.042 $ & $ 1.31\pm 0.246 $&$ 1.38\pm 0.293 $&$ 5.36 $ 
\\
 $\Delta \zeta_{\pi \pi }^\tau(12, 16)$
 & LFQM  & $0.14\pm 0.079 $ & $ 2.43\pm 0.511 $&$ 2.57\pm 0.59 $&$ 5.45 $ 
\\
 & LCSR  & $0.14\pm 0.079 $ & $ 2.76\pm 0.531 $&$ 2.9\pm 0.61 $&$ 4.83 $ 
\\
 $\Delta \zeta_{\pi \pi }^\tau(m_\tau^2, 16)$
 & LFQM  & $0.209\pm 0.117 $ & $ 3.22\pm 0.681 $&$ 3.43\pm 0.797 $&$ 6.09 $ 
\\
 & LCSR  & $0.209\pm 0.117 $ & $ 3.68\pm 0.702 $&$ 3.89\pm 0.818 $&$ 5.37 $ 
\\
\hline
 \hline
\end{tabular} 
\end{center}\end{table}


==> tableBsK.tex <==
\begin{table}[t]
\begin{center}
\caption{Integrated decay widths for
 $B_s\to K^+ \ell\bar  \nu$:
 $\Delta \zeta_K^{\ell} (q_l^2, q_u^2)$. 
Results are given in units of $ps^{-1}$.}
\label{tab:integratedWidthBstoK}
\begin{tabular}{cccccc}
\hline\hline
& LFQM & PQCD & RQM \\\hline
$\Delta \zeta_K^\mu(0, 4)$
 & $1.12\pm 0.099 $&$ 1.36\pm 0.703 $&$ 1.47\pm 0.149 $ 
\\
 $\Delta \zeta_K^\mu(4, 8)$ 
 & $1.17\pm 0.099 $&$ 1.36\pm 0.702 $&$ 1.28\pm 0.135 $ 
\\
$\Delta \zeta_K^\mu(8, 12)$
 & $1.\pm 0.089 $&$ 1.29\pm 0.664 $&$ 1.17\pm 0.116 $ 
\\
$\Delta \zeta_K^\mu(0, 23.77)$
 & $4.18\pm 0.372 $&$ 6.38\pm 3.29 $&$ 6.83\pm 0.688 $ 
\\
\hline
 $\Delta \zeta_K^\tau(m_\tau^2, 8)$
 & $0.551\pm 0.049 $&$ 0.614\pm 0.317 $&$ 0.577\pm 0.058 $ 
\\
$\Delta \zeta_K^\tau(8, 12)$
 & $0.872\pm 0.077 $&$ 1.01\pm 0.516 $&$ 0.894\pm 0.09 $ 
\\
 $\Delta \zeta_K^\tau(m_\tau^2, 23.77)$
 & $2.82\pm 0.25 $&$ 3.95\pm 2.03 $&$ 4.04\pm 0.406 $ 
\\
\hline
$ R_{K}^{\tau/\mu} $
 & 0.675 & 0.619 & 0.592
\\
 \hline\hline
\end{tabular} 
\end{center}\end{table}


==> tableBsKstar.tex <==
\begin{table}[t]
\begin{center}
 \caption{Integrated decay widths for
 $\overline B_s\to K^0 \pi^+  \ell\bar  \nu$:
 $\Delta \zeta_{K\pi}^{\ell} (q_l^2, q_u^2)$.
Results are given in units of $ps^{-1}$.
The S-wave contributions are obtained 
with form factors calculated in the PQCD approach.}
\label{tab:integratedWidthBstoKpi}
\begin{tabular}{cc|cccccccc}
\hline\hline
  & & S-Wave & P-Wave & Total &$f_S(\%)$  \\\hline
$\Delta \zeta_{K\pi}^\mu(0, 4)$
 & LQCD  & $0.278\pm 0.151 $ & $ 1.19\pm 0.151 $&$ 1.47\pm 0.299 $&$ 18.9 $ 
\\
 & LCSR  & $0.278\pm 0.151 $ & $ 1.61\pm 0.172 $&$ 1.89\pm 0.321 $&$ 14.7 $ 
\\
 $\Delta \zeta_{K\pi}^\mu(4, 8)$ 
 & LQCD  & $0.276\pm 0.149 $ & $ 1.58\pm 0.221 $&$ 1.85\pm 0.376 $&$ 14.9 $ 
\\
 & LCSR  & $0.276\pm 0.149 $ & $ 2.13\pm 0.296 $&$ 2.41\pm 0.441 $&$ 11.5 $ 
\\
$\Delta \zeta_{K\pi}^\mu(8, 12)$
 & LQCD  & $0.254\pm 0.137 $ & $ 2.03\pm 0.305 $&$ 2.29\pm 0.436 $&$ 11.1 $ 
\\
 & LCSR  & $0.254\pm 0.137 $ & $ 2.6\pm 0.421 $&$ 2.86\pm 0.552 $&$ 8.88 $ 
\\
$\Delta \zeta_{K\pi}^\mu(12, 16)$
 & LQCD  & $0.202\pm 0.109 $ & $ 2.43\pm 0.347 $&$ 2.63\pm 0.458 $&$ 7.68 $ 
\\
 & LCSR  & $0.202\pm 0.109 $ & $ 2.88\pm 0.505 $&$ 3.08\pm 0.616 $&$ 6.56 $ 
\\
$\Delta \zeta_{K\pi}^\mu(0, 16)$
 & LQCD  & $1.01\pm 0.546 $ & $ 7.22\pm 1.03 $&$ 8.23\pm 1.58 $&$ 12.3 $ 
\\
 & LCSR  & $1.01\pm 0.546 $ & $ 9.23\pm 1.38 $&$ 10.2\pm 1.97 $&$ 9.9 $ 
\\
\hline
 $\Delta \zeta_{K\pi}^\tau(m_\tau^2, 8)$
 & LQCD  & $0.281\pm 0.152 $ & $ 1.36\pm 0.239 $&$ 1.64\pm 0.392 $&$ 17.1 $ 
\\
 & LCSR  & $0.281\pm 0.152 $ & $ 1.7\pm 0.253 $&$ 1.98\pm 0.407 $&$ 14.2 $ 
\\
$\Delta \zeta_{K\pi}^\tau(8, 12)$
 & LQCD  & $0.299\pm 0.162 $ & $ 1.97\pm 0.319 $&$ 2.27\pm 0.48 $&$ 13.2 $ 
\\
 & LCSR  & $0.299\pm 0.162 $ & $ 2.38\pm 0.399 $&$ 2.68\pm 0.56 $&$ 11.2 $ 
\\
 $\Delta \zeta_{K\pi}^\tau(12, 16)$
 & LQCD  & $0.552\pm 0.299 $ & $ 4.32\pm 0.666 $&$ 4.88\pm 0.958 $&$ 11.3 $ 
\\
 & LCSR  & $0.552\pm 0.299 $ & $ 5.09\pm 0.873 $&$ 5.64\pm 1.17 $&$ 9.79 $ 
\\
 $\Delta \zeta_{K\pi}^\tau(m_\tau^2, 16)$
 & LQCD  & $0.834\pm 0.45 $ & $ 5.69\pm 0.895 $&$ 6.52\pm 1.35 $&$ 12.8 $ 
\\
 & LCSR  & $0.834\pm 0.45 $ & $ 6.78\pm 1.14 $&$ 7.62\pm 1.58 $&$ 10.9 $ 
\\
\hline
 \hline
\end{tabular} 
\end{center}
\end{table}

